Privacy Threats Analysis to Secure Federated Learning

Federated learning is emerging as a machine learning technique that trains a model across multiple decentralized parties. It is renowned for preserving privacy as the data never leaves the computational devices, and recent approaches further enhance its privacy by hiding messages transferred in encryption. However, we found that despite the efforts, federated learning remains privacy-threatening, due to its interactive nature across different parties. In this paper, we analyze the privacy threats in industrial-level federated learning frameworks with secure computation, and reveal such threats widely exist in typical machine learning models such as linear regression, logistic regression and decision tree. For the linear and logistic regression, we show through theoretical analysis that it is possible for the attacker to invert the entire private input of the victim, given very few information. For the decision tree model, we launch an attack to infer the range of victim's private inputs. All attacks are evaluated on popular federated learning frameworks and real-world datasets.

==> Makefile <==
# Makefile for LaTeX document files
# Created by Baochun Li, bli@eecg.toronto.edu, March 30 2001
# Modified by Zimu Liu, zimu@eecg.toronto.edu, December 8, 2009
# Last modified: December 8, 2009

# Produce PS/PDF/DVI files: make
# Clean all output files: make clean

# Use pdflatex or latex
ENGINE=pdflatex

# Name of the master LaTeX file
DOCUMENT=main

#--------------------------------------------------
# Do NOT change anything below
#--------------------------------------------------

default: $(DOCUMENT).pdf 

$(DOCUMENT).toc: $(DOCUMENT).tex
	$(ENGINE) $(DOCUMENT).tex

ifeq ($(ENGINE), pdflatex)
#--------------------------------------------------
# pdflatex
#--------------------------------------------------
$(DOCUMENT).pdf: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	$(ENGINE) $(DOCUMENT).tex
	$(ENGINE) $(DOCUMENT).tex

else
#--------------------------------------------------
# latex
#--------------------------------------------------
$(DOCUMENT).dvi: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	$(ENGINE) $(DOCUMENT).tex
	$(ENGINE) $(DOCUMENT).tex

$(DOCUMENT).ps: $(DOCUMENT).dvi
	dvips -t letter -Ppdf -G0 -o $@ $<

$(DOCUMENT).pdf: $(DOCUMENT).ps
	cat $(DOCUMENT).ps | ps2pdf - > $(DOCUMENT).pdf 

endif

all: $(DOCUMENT).pdf $(SUMMARY).pdf

clean:
	rm -rf $(DOCUMENT).aux $(DOCUMENT).log $(DOCUMENT).toc \
  $(DOCUMENT).bbl $(DOCUMENT).blg $(DOCUMENT).pdf \
  $(DOCUMENT).ps $(DOCUMENT).dvi $(DOCUMENT).out \
	*.bak

spell: $(DOCUMENT).tex $/*.tex
	 @ispell -ktexskip1 -t $^


==> review.tex <==
\section{review}


* after Definition 2: "Particularly, if ..." -> In particular, if ...
* "... if N \in R^{m×n} is a Standard Normal Distribution (SND) random variable, every element of N follows the standard normal distribution N (0, 1)." ->In fact, standard normally distributed random variables are often real numbers. It is better to say "We define ..." rather than "If ... then ..."
* "Obviously, N=U_1^{-1}(Z-M)U_2^{-T}." -> you probably mean that N and U_1^{-1}(Z-M)U_2^{-T} follow the same distribution (but what precedes doesn't imply they perfectly correlate)
* "N is a special case that ..." -> N is a special case where ...
* It is common to call an identity n*n matrix I_n, so E_1=I_m and E_2=I_n.
* "the same size of" -> the same size as
* "is transformed into the privacy loss random variable L_{K,X,X}." -> In fact, for every X,X' and K there is a different L_{K,X,X'} and hence (apparently) a different privacy loss random variable. Either the article "the" is not appropriate (there are multiple such variables) or it is better to specify (e.g. "privacy loss random variable corresponding to K,X and X'")
* It is unclear what is exactly the probability distribution of the "privacy loss random variable". The text seems to assume that there is a (hidden) random variable Z on which both P_{K(X)}(Y) and p_{K(X')}(Y) depend in a very specific way. This may be true for the example given, but isn't necessarily true in general. Hence, it would be better to avoid the general statements in the text which are not valid for situations outside the specific case studied. 
* Lemma 1 and 2 are formulated as definitions (rather than as lemmas)

* Lemma 2 has a problem. Here is a counterexample: let \mathbb{X}=\mathbb{Y}=\{-1,+1\}. Let 0<\epsilon<1. Let Z be uniformly distributed over {1,2 ... 100}.
for r,s\in\{-1,+1\}, let f(-1,(r,s)) = r and f(+1,(r,s)) = s. Let Z\in\{-1,+1\} with probability distribution p(Z=(r,s)) = p'(-r).p'(s) with p'(1) = 0.99 and p'(-1)=0.01. Let Y=K(X)=f(X,Z). It follows that p_{K(X)}(X)=0.99 and p_{K(X)}(-X)=0.01. For any X,X'\in\{-1,+1}, if X=X', then we always have L_{K,X,X'}=0 and Eq (4) is satisfied. If X=-X' (assume without loss of generality that X=1 and X'=-1) then we consider the 4 possible values for Z:
-- p(Z=(-1,1)) = 0.99^2; p_{K(X)}(Y)=p_{K(X)}(1)=0.99, p_{K(X')}(Y)=p_{K(X')}(-1)=0.99 => L_{K,X,X'}=0
-- p(Z=(-1,-1)) = 0.0099; p_{K(X)}(Y)=p_{K(X)}(-1)=0.01, p_{K(X')}(Y)=p_{K(X')}(-1)=0.99 => L_{K,X,X'}=-log(99)
-- p(Z=(1,1)) = 0.0099; p_{K(X)}(Y)=p_{K(X)}(1)=0.99, p_{K(X')}(Y)=p_{K(X')}(+1)=0.01 => L_{K,X,X'}=+log(99)
-- p(Z=(1,-1)) = 0.0001; p_{K(X)}(Y)=p_{K(X)}(-1)=0.01, p_{K(X')}(Y)=p_{K(X')}(-1)=0.01 => L_{K,X,X'}=0
As a result, Equation (4) holds true, while obviously this scheme K is not (\epsilon,\delta) differentially private (as with probability 0.99 the private value is returned undisturbed).

* Sec 3.1, after definition 4: "we present an equivalent condition of Eq. 4 for a particular adjacent input pair X, X'" -> Eq (4) didn't require that X and X' were adjacent (but should have done so)

* Lemma 3: "For adjacent input pair X and X'" -> "pair" needs an article
* In the line after Eq (6) : variable B is undefined. In fact, for different values of \delta, the root of g(x)=\delta is different, hence not all these roots can be equal to B.
